A Theorem Prover for Scientific and Educational Purposes

We present a prototype of an integrated reasoning environment for educational purposes. The presented tool is a fragment of a proof assistant and automated theorem prover. We describe the existing and planned functionality of the theorem prover and especially the functionality of the educational fragment. This currently supports working with terms of the untyped lambda calculus and addresses both undergraduate students and researchers. We show how the tool can be used to support the students' understanding of functional programming and discuss general problems related to the process of building theorem proving software that aims at supporting both research and education.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{P. Quaresma and W. Neuper (Eds.): 6th International Workshop\\ on Theorem proving components for Educational software (ThEdu'17)\\
EPTCS 267, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.267.4}{10.4204/EPTCS.267.4}}
\pdfoutput=1

